Single-cell RNA-seq data imputation using Feature Propagation

While single-cell RNA sequencing provides an understanding of the transcriptome of individual cells, its high sparsity, often termed dropout, hampers the capture of significant cell-cell relationships. Here, we propose scFP (single-cell Feature Propagation), which directly propagates features, i.e., gene expression, especially in raw feature space, via cell-cell graph. Specifically, it first obtains a warmed-up cell-gene matrix via Hard Feature Propagation which fully utilizes known gene transcripts. Then, we refine the k-Nearest Neighbor(kNN) of the cell-cell graph with a warmed-up cell-gene matrix, followed by Soft Feature Propagation which now allows known gene transcripts to be further denoised through their neighbors. Through extensive experiments on imputation with cell clustering tasks, we demonstrate our proposed model, scFP, outperforms various recent imputation and clustering methods. The source code of scFP can be found at https://github.com/Junseok0207/scFP.

==> deprecated/scFP_old.tex <==
% %%%%%%%% ICML 202 EXAMPLE LATEX SUBMISSION FILE %%%%%%%%%%%%%%%%%

% \documentclass[nohyperref]{article}

% % Recommended, but optional, packages for figures and better typesetting:
% \usepackage{microtype}
% \usepackage{graphicx}
% \usepackage{subfigure}
% \usepackage{booktabs} % for professional tables

% % hyperref makes hyperlinks in the resulting PDF.
% % If your build breaks (sometimes temporarily if a hyperlink spans a page)
% % please comment out the following usepackage line and replace
% % \usepackage{icml2023} with \usepackage[nohyperref]{icml2023} above.
% \usepackage{hyperref}
% \usepackage{algpseudocode}
% \usepackage{capt-of}% or \usepackage{caption}

% % Attempt to make hyperref and algorithmic work together better:
% \newcommand{\theHalgorithm}{\arabic{algorithm}}
% \newcommand{\proposed}{\text{scFP}}

% % Use the following line for the initial version submitted for review:
% \usepackage{icml2023}

% % If accepted, instead use the following line for the camera-ready submission:
% % \usepackage[accepted]{icml2023}

% % For theorems and such
% \usepackage{amsmath}
% \usepackage{amssymb}
% \usepackage{mathtools}
% \usepackage{amsthm}

% % if you use cleveref..
% \usepackage[capitalize,noabbrev]{cleveref}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % THEOREMS
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \theoremstyle{plain}
% \newtheorem{theorem}{Theorem}[section]
% \newtheorem{proposition}[theorem]{Proposition}
% \newtheorem{lemma}[theorem]{Lemma}
% \newtheorem{corollary}[theorem]{Corollary}
% \theoremstyle{definition}
% \newtheorem{definition}[theorem]{Definition}
% \newtheorem{assumption}[theorem]{Assumption}
% \theoremstyle{remark}
% \newtheorem{remark}[theorem]{Remark}

% % Todonotes is useful during development; simply uncomment the next line
% %    and comment out the line below the next line to turn off comments
% %\usepackage[disable,textsize=tiny]{todonotes}
% \usepackage[textsize=tiny]{todonotes}


% % The \icmltitle you define below is probably too long as a header.
% % Therefore, a short form for the running title is supplied here:
% % \icmltitlerunning{Single-Cell RNA-seq denoising using Feature Propagation}

% \begin{document}

% \twocolumn[
% \icmltitle{Denoising single-cell RNA-seq data using Feature Propagation}


% % List of affiliations: The first argument should be a (short)
% % identifier you will use later to specify author affiliations
% % Academic affiliations should list Department, University, City, Region, Country
% % Industry affiliations should list Company, City, Region, Country

% % You can specify symbols, otherwise they are numbered in order.
% % Ideally, you should not use this facility. Affiliations will be numbered
% % in order of appearance and this is the preferred way.
% \icmlsetsymbol{equal}{*}

% \begin{icmlauthorlist}
% \icmlauthor{Firstname1 Lastname1}{equal,yyy}
% \icmlauthor{Firstname2 Lastname2}{equal,yyy,comp}
% \icmlauthor{Firstname3 Lastname3}{comp}
% \icmlauthor{Firstname4 Lastname4}{sch}
% \icmlauthor{Firstname5 Lastname5}{yyy}
% \icmlauthor{Firstname6 Lastname6}{sch,yyy,comp}
% \icmlauthor{Firstname7 Lastname7}{comp}
% %\icmlauthor{}{sch}
% \icmlauthor{Firstname8 Lastname8}{sch}
% \icmlauthor{Firstname8 Lastname8}{yyy,comp}
% %\icmlauthor{}{sch}
% %\icmlauthor{}{sch}
% \end{icmlauthorlist}

% \icmlaffiliation{yyy}{Department of XXX, University of YYY, Location, Country}
% \icmlaffiliation{comp}{Company Name, Location, Country}
% \icmlaffiliation{sch}{School of ZZZ, Institute of WWW, Location, Country}

% \icmlcorrespondingauthor{Firstname1 Lastname1}{first1.last1@xxx.edu}
% \icmlcorrespondingauthor{Firstname2 Lastname2}{first2.last2@www.uk}

% % You may provide any keywords that you
% % find helpful for describing your paper; these are used to populate
% % the "keywords" metadata in the PDF but will not be shown in the document
% \icmlkeywords{Machine Learning, ICML}

% \vskip 0.3in
% ]

% % this must go after the closing bracket ] following \twocolumn[ ...

% % This command actually creates the footnote in the first column
% % listing the affiliations and the copyright notice.
% % The command takes one argument, which is text to display at the start of the footnote.
% % The \icmlEqualContribution command is standard text for equal contribution.
% % Remove it (just {}) if you do not need this facility.

% %\printAffiliationsAndNotice{}  % leave blank if no need to mention equal contribution
% \printAffiliationsAndNotice{\icmlEqualContribution} % otherwise use the standard text.

% \begin{abstract}
% While single-cell RNA sequencing provides an understanding of the transcriptome of individual cells, its high sparsity, often termed dropout, hampers the capture of significant cell-cell relationships. Here, we propose \proposed~(single-cell Feature Propagation), which directly propagates features, i.e., gene expression, especially in raw feature space, via cell-cell graph. Specifically, it first obtains a warmed-up cell-gene matrix via Hard Feature Propagation which fully utilizes known gene transcripts. Then, we refine the $k$-Nearest Neighbor ($k$NN) of the cell-cell graph with a warmed-up cell-gene matrix, followed by Soft Feature Propagation which now allows known gene transcripts to be further denoised through their neighbors. Through extensive experiments on imputation with cell clustering tasks, we demonstrate our proposed model,~\proposed, outperforms various recent imputation and clustering methods. The codes can be found on \url{https://github.com/Junseok0207/scFP/}.
% \end{abstract}

% \section{Introduction}
% % 1. 기존 dropout 문제 언급
% Single-cell RNA-sequencing (scRNA-seq) analysis has attracted significant attention due to its property to profile transcriptome-wide gene expression at single-cell resolution. It provides researchers opportunities to perform various analyses, including the identification of new cell types, inferring cell trajectories, and the discovery of intercellular signaling pathways. However, the analysis of scRNA-seq data can be challenging due to the noisy nature of the observed expression value. Specifically, scRNA-seq data often suffer from low transcript capture, referred to as dropout phenomena~\cite{dropout}, which causes the occurrence of false zero values. Furthermore, the observed non-zero expression values also suffer from biologically irrelevant signals, such as batch effects~\cite{batcheffect} and transcriptional noise~\cite{noise}.

% Many works have been proposed to denoise the scRNA-seq data by imputing the given expression values. Among them, smoothing-based methods assume that cells with similar expression profiles are likely to share similar underlying biological characteristics. By leveraging this assumption, these methods impute gene expression values by forcing the expression values of neighboring cells to be more similar. Specifically, DrImpute~\cite{drimpute} averages the expression values based on a pre-calculated cluster, and MAGIC~\cite{magic}~performs a diffusing process on the calculated Markov affinity-based graph. Despite the simple architecture, these methods are effective in reducing noise from various factors. However, there are some limitations to be considered: 1) it can decrease the meaningful cell variability by smoothing expression values across incorrect cell groups when neighboring cells are misdefined, and 2) noise expression values could be spread during smoothing when the observed expression values are noisy, which can be severe if it contains many false zero values due to the dropout phenomena.

% Recently, most researchers are focused on the imputation methods that utilize deep neural networks (DNNs) to reconstruct gene expressions. These lines of methods utilize an autoencoder architecture, where the cell representation is learned through an encoder, and then impute values by passing them through the decoder layer. Specifically, DCA~\cite{dca} reconstructs the gene expression by assuming zero-inflated negative binomial (ZINB) distribution and AutoClass~\cite{autoclass} further learns the classifier by providing pseudo-labels generated by pre-clustering. Furthermore, scGCL~\cite{scgcl}, inspired by AFGRL~\cite{afgrl}, leverages relationship information between cells using graph neural networks (GNNs) on a cell-cell graph and learns cell representations in a self-supervised manner. However, despite their complex modeling, the output of these methods often shows poor performance on the subsequent downstream tasks compared to that of raw expression values. We argue that this is because effectively optimizing complex DNN models on a given dataset requires appropriate hyper-parameter choices, which can be challenging in the context of imputation tasks due to the unsupervised nature.

% In this paper, we propose a simple but effective imputation method, named~\proposed, for denoising observed scRNA-seq data with a bi-level feature propagation scheme. Specifically, we first impute the zero values using the feature propagation scheme on the initially defined $k$NN graph while preserving the non-zero values that contain relatively lower noise (Sec~\ref{sec:hard_fp}) to prevent the contamination of biological signals from prevalent false zero values. Using this warmed-up data, the $k$NN graph is further refined to capture the correct neighbors of each cell, after which we pass it through another feature propagation module that also changes the value of non-zero values (Sec~\ref{sec:soft_fp}) to denoise the bias or noise on these values. Through experiments on both real and simulated scRNA-seq datasets, we demonstrate the effectiveness of~\proposed.

% \begin{figure*}[!t]
% 	\centering
% 	\includegraphics[width=1\textwidth]{imgs/main_new_cropped.pdf}
%         \vspace{-5ex}
%         \caption{The overall architecture of \proposed.}
%         \label{fig:architecture}
%         \vspace{-3ex}
% \end{figure*}

% \section{Methods}

% \noindent{\textbf{Notation.}} Given a cell-gene feature matrix, $\mathbf{X} \in \mathbb{R}^{N\times M}$, where $N$ and $M$ denote the number of cells and genes, respectively, let $\mathcal{G}=(\mathcal{V},\mathcal{E},\mathbf{X})$ denote a cell-cell graph. $\mathcal{V}=\{v_1,...,v_N\}$ denotes the set of cell nodes, $\mathcal{E} \subseteq \mathcal{V} \times \mathcal{V}$ denotes the set of edges, $\mathbf{A} \in \mathbb{R}^{N \times N}$ denotes an adjacency matrix where $\mathbf{A}_{ij}=1$ iff $(v_i, v_j) \in \mathcal{E}$ and $\mathbf{A}_{ij}=0$ otherwise. Additionally, we denote $\tilde{\textbf{A}}=\mathbf{D}^{-1/2}\mathbf{A}\mathbf{D}^{-1/2}$ as a symmetrically normalized adjacency and represent graph laplacian matrix $\Delta=\mathbf{I}-\tilde{\mathbf{A}}$ where $\mathbf{I}$ is an identity matrix.

% % \noindent{\textbf{Notation.}} Given a cell-gene feature matrix, $\mathbf{X} \in \mathbb{R}^{N\times M}$, where $N$ and $M$ denote the number of cells and genes, respectively, let $\mathcal{G}=(\mathcal{V},\mathcal{E},\mathbf{X})$ denote a cell-cell graph. $\mathcal{V}=\{v_1,...,v_N\}$ denotes set of cell nodes, $\mathcal{E} \subseteq \mathcal{V} \times \mathcal{V}$ denotes set of edges, $\mathbf{A} \in \mathbb{R}^{N \times N}$ denotes an adjacency matrix where $\mathbf{A}_{ij}=1$ iff $(v_i, v_j) \in \mathcal{E}$ and $\mathbf{A}_{ij}=0$ otherwise.

% \subsection{Preliminary: Feature Propagation}

% Recently, Feature Propagation (FP) \cite{fp} has been introduced to mitigate missing features in graph domain. The core idea of FP is to diffuse the features that we know, i.e., provided, to the features that we do not know, i.e., missing, while maintaining the initial state of known features. Formally, given a node feature matrix, consisting of $k$ known features and $u$ unknown features in each feature dimension, i.e., $f$, heat diffusion equation at time step $t$ can be expressed as:
% \vspace{-2ex}
% \begin{equation}
% \label{eqn:heat_diffusion}
% \begin{gathered}
% \dot{\mathbf{X}}(t)=-\Delta \mathbf{X}(t), \\
% (\text{IC}) \mathbf{X}_{\cdot,f}(0)=\left[\begin{array}{c} \small \mathbf{X}_{k,f}\\ \mathbf{X}_{u,f}(0)\end{array}\right], 
% (\text{BC}) \mathbf{X}_{k,f}(t)=\mathbf{X}_{k,f}, \\
% % \forall k_{f} \in \mathcal{V}_{known,f}, \forall u_{f} \in \mathcal{V}_{unknown,f}, \forall f \leq F
% \forall k \in \mathcal{V}_{k,f}, \forall u \in \mathcal{V}_{u,f}, \forall f \leq F
% \end{gathered}
% \end{equation}
% % \vspace{-12ex}
% \noindent where $\mathbf{X}_{\cdot,f}\in \mathbb{R}^N$ denotes feature vector at dimension $f$ bounded by $F$, (IC) and (BC) denotes initial conditions and boundary conditions, respectively. $\mathcal{V}_{k,f}$ and $\mathcal{V}_{u,f}$ denotes a set of \textit{known} nodes and \textit{unknown} nodes at feature dimension, $f$, respectively. Here, solving Equation~\ref{eqn:heat_diffusion} by linear equation, we obtain closed-from solution, $\mathbf{X}_{u}=-\Delta_{uu}^{-1}\Delta_{ku}^{\top}\mathbf{X}_{k}$. However, during calculation, it induces complexity of $\mathcal{O}(|\mathcal{V}_{u}|^3)$, which is not desirable in large graphs. Thus, we resort to an iterative Euler scheme and derive a formula as follows:
% \begin{equation}
% \label{eqn:iterative}
% \mathbf{X}^{(i+1)}=\left[\begin{array}{cc}
% \mathbf{I} & \mathbf{0} \\
% \tilde{\mathbf{A}}_{uk} & \tilde{\mathbf{A}}_{uu}
% \end{array}\right] \mathbf{X}^{(i)}
% \end{equation}
% \noindent where $\mathbf{X}^{(i)}$ represents imputed feature matrix at $i$ step. It is important to note that this formula is basically equivalent to multiplying the feature matrix with normalized adjacency while maintaining known feature values as its initial state. It shows the robust performance in the graph domain even when the data contains more than 90\% missing features~\cite{fp}. However, it cannot be naively applied to scRNA-seq data due to its following inherent nature: 1) The information regarding which features are missing or noisy is unknown. 2) Since graph structure is not provided, it is crucial to construct a graph that connects biologically relevant cells.

% % 그래프 정보 주어지지 않아서 우리가 직접 만들어야하는 단점. (이게 크리티컬 하고)
% % 그리고 feature matrix 측면에서도 graph 는 대부분 0, 1로 binary 하게 분류하고 0 자체를 certain 한 missing으로 봄. 우리는 값이 count matrix 에서 비롯돼서 발현되는 값들 사이에서도 variance 가 있고 0 인 애들이 dropout 이라는 특수한 상황을 마주하고 있어서 특별하게 adopation 을 해야만 하는 상황.

% \subsection{Proposed Methodology: \proposed}
% We propose the bi-level feature propagation method that extends FP in a manner that is well-suited to the scRNA-seq domain. Our overall architecture can be found in Figure~\ref{fig:architecture}. We first define a cell-cell graph using observed scRNA-seq data and perform a diffusion process using a Hard Feature Propagation scheme (Sec~\ref{sec:hard_fp}) that primarily pays attention to denoising zero values in the cell-gene count matrix while preserving non-zero values. After that, we refine the cell-cell graph by calculating $k$-nearest neighbors for each cell using the previously smoothed outputs (i.e., warmed-up data). Then, we pass through Soft Feature Propagation (Sec~\ref{sec:soft_fp}) which allows the denoising of observed gene transcripts. Detail about each component can be found in the following sections.

% % \noindent{\textbf{Task: Downstream Task based on Denoised Cell-Gene Matrix.}} Given a sparse and noisy cell-gene matrix, $\mathbf{X}$, we aim to obtain a denoised cell-gene matrix, $\tilde{\mathbf{X}}$ which is well suited for downstream tasks in the scRNA-seq domain.

% \subsubsection{Hard Feature Propagation}
% \label{sec:hard_fp}
% We start with imputing zero values, i.e., dropouts in gene expression with the aid of similar cells. To do so, we first need to define an adjacency matrix which first brings us a challenge compared to the graph domain, where adjacency information is provided. Here, the intuitive and cheap way that facilitates message-passing between similar cells is to introduce a $k$NN graph by calculating cosine similarities. However, considering the sparsity of cell-gene matrix \cite{magic, misc}, which is a direct resource for building $k$NN graph, we argue that obtained $k$NN graph should merely serve as an initialized graph for warming-up sparse and noisy gene transcripts. In this regard, as our primal goal is to denoise zero-valued gene expressions, we apply Hard Feature Propagation as follows:
% \begin{equation}
% \label{eqn:hard_fp}
% \mathbf{X}^{(i+1)}=\left[\begin{array}{cc}
% \mathbf{I} & \mathbf{0} \\
% \tilde{\mathbf{A}}_{uk}^{\text{initial}} & \tilde{\mathbf{A}}_{uu}^{\text{initial}}
% \end{array}\right] \mathbf{X}^{(i)}
% \end{equation}
% \noindent where $\mathbf{X}^{(i)} \in \mathbb{R}^{N\times M}$ represents imputed cell-gene feature matrix at step $i$. After that, we obtain a converged warm-up matrix, $\mathbf{X}^{(K)}$, which is now denser and smoothed via neighbors. 
% Note that in this step, we employ a hard clamping strategy where the non-zero values, which correspond to the observed expression values, are retained at their original values.
% This is because, in this step, more emphasis is placed on denoising zero-values, which are more prevalent in the cell-gene count matrix, compared to denoising non-zero transcript values. This is because non-zero values generally contain less noise than zero-values.

% % It is important to note that, at this moment, we used a hard clamping technique to known values, i.e., expressed genes, where known values maintain their initial values. 

% % This is because in the denoising zero-values, which is more prevalent in the cell-gene count matrix, has more priority than denoising non-zero transcripted values since the latter generally contains less noise than that of zero-values.

% %possess much more certainty than those of zero-values.


% \subsubsection{Refining Cell-Cell Graph}
% With a warmed-up cell-gene matrix, $\mathbf{X}^{(K)}$ originating from Hard Feature Propagation, we make use of this matrix to refine an initial cell-cell graph which was built when cell representation was sparse. More precisely, a warmed-up cell-gene matrix is used as input for $k$NN graph as follows:
% \begin{equation}
% \label{eqn:refine}
% % \begin{gathered}
% \tilde{\mathbf{A}}^{\text{refined}} = k\text{NN}(\mathbf{X}^{(K)})
% % \end{gathered}
% \end{equation}
% \noindent where $\tilde{\mathbf{A}}^{\text{refined}} \in \mathbb{R}^{N\times N}$ is refined normalized adjacency for a cell-cell graph which is built considering the denoised zero-values, which was not feasible to capture in the initial stage of $k$NN graph generation. In other words, this process could potentially reveal hidden or implicit graph structures that were not initially detectable due to sparse and noisy gene expression. We argue that this refined adjacency matrix may provide more accurate or robust graph representations, which could enhance subsequent analyses or learning tasks.

% \subsubsection{Soft Feature Propagation}
% \label{sec:soft_fp}
% Here, equipped with warmed-up cell-gene matrix, $\mathbf{X}^{(K)}$ and refined adjacency matrix for cell-cell graph, $\tilde{\mathbf{A}}^{\text{refined}}$, we now run Soft Feature Propagation. Specifically, compared to Hard Feature Propagation which is based on hard clamping \cite{lp_main, lp_var3, lp_var4}, at this moment, we rather adopt soft clamping \cite{lp_var1, lp_var2}, which basically leaves room for updating the originally transcripted gene value of its neighbors endowed with implicit graph structures thanks to the warmed-up procedure. This aligns with our motivation to take into account noise from not only low transcript capture but also from the observed non-zero expression values that might possess biologically irrelevant signals, e.g., batch effects and transcriptional noise~\cite{batcheffect, noise}. Formally, Soft Feature Propagation is applied as follows:
% \begin{equation}
% \label{eqn:soft}
% % \begin{gathered}
% \mathbf{X}^{(K+j+1)} = \alpha\tilde{\mathbf{A}}^{\text{refined}}\mathbf{X}^{(K+j)}+(1-\alpha)\mathbf{X}^{(K)}
% % \end{gathered}
% \end{equation}
% \noindent where $\mathbf{X}^{(K+j)}$ is the updated cell-gene matrix at step $j$, $0<\alpha<1$ is the constant\footnote{As we aim to denoise known values, i.e., not to maintain its original state, we fixed $\alpha$ as 0.99 and used as constant.} that controls amount of information that $\mathbf{X}^{(K+j)}$ receives from its neighbors. After another $K$ iteration, we finally obtain a converged and denoised cell-gene matrix, $\tilde{\mathbf{X}} = \mathbf{X}^{(2K)}$ that takes into account both the noise from zero-values, i.e., dropout and noise from observed non-zero expression values, e.g., transcriptional noise. Overall implementation details can be found in Appendix~\ref{implementation details} with pseudo-code.


% % With this in mind, scFP can seamlessly be incorporated as a preprocessing module in any existing work. Overall, in this work, we aim to emphasize simple and straightforward ways to enhance performance in imputation and clustering tasks. We hope our straightforward yet efficient algorithm can serve as a new robust baseline and contribute to advancements in the single-cell RNA sequencing field.



% \begin{table*}[t]
% \caption{Overall performance in imputation task measured by RMSE.}
% \centering  
% \label{table:imputation}
% \begin{small}
% % \begin{sc}
% \resizebox{0.7\textwidth}{!}{
% \begin{tabular}{c|ccc|ccc|ccc|ccc|ccc}
% \toprule
%               & \multicolumn{3}{c|}{Baron Mouse}   & \multicolumn{3}{c|}{Mouse ES}      & \multicolumn{3}{c|}{Mouse Bladder} & \multicolumn{3}{c|}{Zeisel}        & \multicolumn{3}{c}{Baron Human}   \\ \cline{2-16} 
%               & \multicolumn{3}{c|}{Dropout Rates} & \multicolumn{3}{c|}{Dropout Rates} & \multicolumn{3}{c|}{Dropout Rates} & \multicolumn{3}{c|}{Dropout Rates} & \multicolumn{3}{c}{Dropout Rates} \\ \cline{2-16} 
%               & 20\%        & 40\%        & 80\%      & 20\%        & 40\%        & 80\%      & 20\%        & 40\%       & 80\%       & 20\%        & 40\%       & 80\%       & 20\%        & 40\%       & 80\%      \\ \hline
% MAGIC         & 0.61       & 0.73       & 0.99     & 0.53       & 0.73       & 1.21     & 0.50       & 0.60      & 0.82      & 0.60       & 0.82      & 1.31      & 0.58       & 0.74      & 1.06     \\
% DCA           & 0.42       & 0.43       & 0.49     & 0.35       & 0.35       & 0.36     & 0.37       & 0.38      & 0.41      & 0.39       & 0.42      & 0.44      & 0.41       & 0.43      & 0.47     \\
% AutoClass     & 0.63       & 0.76       & 0.98     & 0.53       & 0.75       & 1.23     & 0.52       & 0.64      & 0.82      & 0.60       & 0.84      & 1.32      & 0.59       & 0.76      & 1.08     \\
% scGCL         & 0.64       & 0.74       & 0.97     & 0.59       & 0.75       & 1.16     & 0.51       & 0.62      & 0.81      & 0.66       & 0.82      & 1.29      & 0.63       & 0.77      & 1.08     \\ \hline
% scFP (Ours)          & \textbf{0.36}       & \textbf{0.37}       & \textbf{0.43}     & \textbf{0.32}       & \textbf{0.32}       & \textbf{0.36}    & \textbf{0.26}       & \textbf{0.26}      & \textbf{0.31}      & \textbf{0.39}       & \textbf{0.40}      & \textbf{0.44}      & \textbf{0.33}       & \textbf{0.34}      & \textbf{0.39}   \\
% \bottomrule
% \end{tabular}
% }
% % \end{sc}
% \end{small}
% \end{table*}

% % \vspace{-3ex}

% \begin{table*}[t]
% \caption{Overall performance of cell clustering task measured by ARI, NMI, CA.}
% \centering
% \label{table:cell_clustering}
% \begin{small}
% % \begin{sc}
% \resizebox{0.7\textwidth}{!}{
% \begin{tabular}{c|ccc|ccc|ccc|ccc|ccc}
% \toprule
%               & \multicolumn{3}{c|}{Baron Mouse} & \multicolumn{3}{c|}{Mouse ES} & \multicolumn{3}{c|}{Mouse Bladder} & \multicolumn{3}{c|}{Zeisel} & \multicolumn{3}{c}{Baron Human} \\ \cline{2-16} 
%               & ARI       & NMI       & CA       & ARI      & NMI      & CA      & ARI        & NMI       & CA        & ARI     & NMI     & CA      & ARI       & NMI      & CA       \\ \hline
% Raw           & 0.44      & 0.71      & 0.56     & 0.74     & 0.75     & 0.79    & 0.59       & 0.75      & 0.68      & 0.70    & 0.75    & 0.77    & 0.44      & 0.71     & 0.56     \\
% MAGIC         & 0.42      & 0.72      & 0.57     & 0.80     & \textbf{0.85}     & 0.83    & 0.55       & 0.75      & 0.64      & 0.70    & 0.75    & 0.76    & 0.56      & 0.78     & 0.59     \\
% DCA           & 0.46      & 0.69      & 0.59     & 0.76     & 0.78     & 0.81    & 0.39       & 0.59      & 0.54      & 0.67    & 0.72    & 0.75    & 0.53      & 0.74     & 0.55     \\
% AutoClass     & 0.44      & 0.71      & 0.52     & 0.74     & 0.75     & 0.81    & 0.51       & 0.75      & 0.64      & 0.71    & 0.75    & 0.77    & 0.44      & 0.71     & 0.52     \\
% scGCL         & 0.43      & 0.72      & 0.54     & 0.73     & 0.75     & 0.79    & 0.53       & 0.75      & 0.64      & 0.65    & 0.70    & 0.73    & 0.50      & 0.78     & 0.62     \\
% kNN-smoothing & 0.43      & 0.72      & 0.55     & 0.72     & 0.74     & 0.79    & 0.59       & 0.76      & 0.68      & 0.68    & 0.73    & 0.76    & 0.56      & 0.78     & 0.56     \\ \hline
% scFP (Ours)          & \textbf{0.61}      & \textbf{0.82}      & \textbf{0.76}     & \textbf{0.82}     & 0.83     & \textbf{0.85}    & \textbf{0.65}       & \textbf{0.77}      & \textbf{0.73}      & \textbf{0.85}    & \textbf{0.81}    & \textbf{0.89}    & \textbf{0.68}     & \textbf{0.83}     & \textbf{0.73}    \\
% \bottomrule
% \end{tabular}
% }
% % \end{sc}
% \end{small}
% \end{table*}

% \section{Experiments}

% \noindent\textbf{Experimental Settings. } To evaluate the effectiveness of~\proposed, we evaluated~\proposed~with 5 widely used real-world scRNA-seq data, Baron Mouse, Mouse ES, Mouse Bladder, Zeisel, and Baron Human. The detailed statistics of these datasets can be found in Appendix~\ref{appendix:statistics}.


% \noindent\textbf{Performance on Imputation. } Table~\ref{table:imputation} shows the overall performance in imputation tasks with dropout rates ranging from the low case, e.g., 20\%, to the severe case, e.g., 80\%. We observe~\proposed~shows robust performance regardless of dropout rates outperforming other baselines designed for denoising cell-gene matrix. Among baselines, it is worth noting that more complex models, e.g., AutoClass, and scGCL, exhibit lower performance than DCA. This tells us that the complexity of the model does not always guarantee denoising performance in the scRNA-seq domain. In this regard, as~\proposed~does not equip any learnable parameters, propagating features on the raw feature space while carefully handling observed values is an intuitive and effective way to obtain a denoised cell-gene matrix.
% % DCA performed relatively well, and we argue that this performance gain was feasible due to the introduction of ZINB distribution, which takes into account the dropout phenomenon. Other DNN-based approaches could not avoid its deterioration as dropout rates get severe, e.g., 80\%.


% % While other DNN-based approaches, e.g., AutoClass and scGCL, take similar approaches in order to denoise dropouts, the complex model optimization could not benefit in such harsh dropout cases, e.g., 80\% facing its deterioration. Although MAGIC propagates features based on Markov Affinity, the lack of ability to differently handle originally observed feature values, e.g., maintaining its initial state, 

% \noindent\textbf{Performance on Cell Clustering. } Now, with obtained denoised cell-gene matrix, we further evaluate whether the denoised matrix performs well on the representative downstream task, cell clustering. As shown in Table~\ref{table:cell_clustering}, we observe~\proposed~achieve promising results in terms of Adjusted Rand Index (ARI), Normalized Mutual Information (NMI), and Clustering Accuracy (CA). Interestingly, while DCA performed well on imputation tasks compared to other baselines, its robustness could not be maintained in clustering tasks. It is also worth noting that \proposed~consistently outperforms the performance of MAGIC, demonstrating that the bi-level feature propagation and structure refinement are important to effectively denoise the scRNA-seq data. Furthermore,~\proposed~demonstrates its robustness by consistently exhibiting superior performance compared to raw data across all five datasets.



% % Interestingly, while DCA performed well on imputation tasks compared to other baselines, its robustness could not be maintained in clustering tasks. 
% % Specifically, in Mouse Bladder, it eventually fails more than the simple baseline, Raw, which processes clustering solely based on the input cell-gene matrix. Such a tendency tells us a well-denoised matrix that does not always guarantee performance at subsequent downstream tasks. However,~\proposed~maintained its robust performance even at the downstream task, telling us ~\proposed~denoise the cell-gene matrix in an appropriate way that is well-suited for following downstream tasks.

% \noindent\textbf{Ablation studies. } Here, we conduct ablation studies from two perspectives, as demonstrated in Figure~\ref{fig:ablation}. First, by incremental ablation on each module, we observe~\proposed~fully benefits when feature propagation has been made in both Hard and Soft ways. Here, it is important to note that utilizing a refined $k$NN graph, where a graph is reconstructed by a warmed-up matrix, is crucial before processing Soft Feature Propagation. Also, with ablation on the sequence of Feature Propagation, we verify the usage of Hard Feature Propagation, which maintains the observed value with its initial state at the early stage of denoising is significant. However, solely resorting to Hard Feature Propagation outputs sub-optimal results since it does not leave room for the observed values, which also possess the possibility of being noisy, to be denoised via their neighbors.


% \begin{figure}[h]
% 	\centering
% 	\includegraphics[width=0.45\textwidth]{imgs/ablation_new_cropped.pdf}
%         \vspace{-2ex}
%         \caption{Ablation Studies of~\proposed. (a) "Hard+Soft+Refine $k$NN" corresponds to~\proposed. (b) "Hard$\rightarrow$Soft" corresponds to~\proposed. Zeisel dataset is used.}
%         \label{fig:ablation}
%         \vspace{-1ex}
% \end{figure}


% \noindent\textbf{Simulation studies. }
% To demonstrate our claim that the diffusion of noise from false zeros can have a negative effect, we conducted experiments using a simulation dataset generated by Splatter Package~\cite{splatter}, where we can control the dropout rate, indicating the proportion of zero values. In Figure~\ref{fig:tsne}, MAGIC, which diffuses both zero and non-zero values, successfully separates cell types by preserving biologically relevant signals even in situations where raw features are noisy when the dropout rate is relatively low (i.e., 22.13\%). However, in cases with a high dropout rate (i.e., 56.65\%), where there are many false zeros, it fails to separate cell types because of the noisy diffusion. On the other hand, \proposed~effectively separates cell types even in situations with a high dropout rate by reducing the noise in the false zero signal through the Hard FP step.


% \begin{figure}[t]
% 	\centering
% 	\includegraphics[width=0.7\linewidth]{imgs/TSNE.eps}
%          \vspace{-2.5ex}
%         \caption{t-SNE visualization result on simulated dataset over various dropout rates. The rates at the top represent the dropout rate, which equals to the proportion of false zero values.}
%         \vspace{-3ex}
%         \label{fig:tsne}
% \end{figure}



% \section{Conclusion}
% In this paper, we proposed~\proposed~which denoises the observed scRNA-seq data that is inherently sparse and noisy. Specifically, we first aimed to denoise zero-values of transcripts in Hard Feature Propagation with hard clamping of observed values. With a warmed-up matrix, we then refined the $k$NN graph and proceeded with Soft Feature Propagation in order to denoise known values with its neighbors, taking into account the potential of transcriptional noise. With a simple and lightweight design, its imputation and cell clustering performance under various datasets verifies the effectiveness of~\proposed. 

% \clearpage
% \bibliography{scFP_reference}
% \bibliographystyle{icml2023}


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % APPENDIX
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \newpage
% \appendix
% \onecolumn


% \section{Data statistics}
% \label{appendix:statistics}

% \label{sec:data_statistics}
% \begin{table}[h]
% \centering
% % \small
% \caption{Statistics for real datasets used for experiments.}
% %\renewcommand{\arraystretch}{1.0}
% %\resizebox{\linewidth}{!}
% \resizebox{0.6\linewidth}{!}{
% \begin{tabular}{c|ccccc}
% \noalign{\smallskip}\noalign{\smallskip}
% \toprule
% Data & \# of Cells & \# of Genes & \# of Subgroups \\
% \hline
% Baron Mouse & 1,886 & 14,861 & 13 \\
% Mouse ES cells & 2,717 & 24,047 & 4 \\
% Mouse bladder cells & 2,746 & 19,771 & 16 \\
% Zeisel & 3,005 & 19,972 & 9 \\
% Baron Human & 8,569 & 20,125 & 14 \\
% Shekhar mouse retina cells & 27,499 & 13,166 & 19 \\
% \bottomrule
% \end{tabular}
% }
% \label{tab:real dataset}
% \end{table}











% \section{Extension to large dataset}

% \begin{table*}[h]
% \begin{minipage}{0.45\linewidth}{
%     \centering
%     \small
%     \caption{Performance of cell clustering in Shekhar Mouse Retina dataset}
%     % \vspace{-2ex}
%     \resizebox{0.9\linewidth}{!}{
%         \begin{tabular}{c|ccc}
%         \bottomrule
%                       & \multicolumn{3}{c}{Shekhar mouse retina} \\ \cline{2-4} 
%                       & ARI     & NMI     & CA      \\ \hline
%         Raw           & 0.54    & 0.76    & 0.61    \\
%         MAGIC         & 0.80    & 0.85    & 0.83    \\
%         DCA           & 0.34    & 0.37    & 0.42    \\
%         AutoClass     & 0.74    & 0.75    & 0.81    \\
%         scGCL         & 0.54    & 0.74    & 0.58    \\
%         kNN-smoothing & 0.47    & 0.75    & 0.55    \\ \hline
%         scFP (Ours)         & \textbf{0.91}    & \textbf{0.83}    & \textbf{0.82}   \\
%         \bottomrule
%         \end{tabular}
%         }
%     \label{tab:bi_table}
% } \end{minipage}
% \begin{minipage}{0.5\linewidth}{
% \centering
%     \includegraphics[width=0.8\linewidth]{imgs/ablation_new_large_cropped.pdf} % Reduce the figure size so that it is slightly arrower than the column. Don’t use precise values for figure width.This setup will avoid overfull boxes.
%     \vspace{-2ex}
%     \captionof{figure}{Ablation of each module inf~\proposed~in Shekhar Mouse Retina dataset. "$\text{Hard}\text{+}\text{Soft}\text{+}\text{Refine $k$NN}$" denotes~\proposed.}
%     \label{fig:bi_figure}
% }\end{minipage}
% % \vspace{-2ex}
% \end{table*}


% Here, we further extended our experiment on a relatively large dataset, Shekhar mouse retina cells, and compared the performance of cell clustering in Table~\ref{tab:bi_table} with its ablation study on each module on~\proposed. Despite the absence of trainable parameters, our proposed method still demonstrates promising clustering performance on a large dataset. This suggests that, sometimes, rather than focusing on the complexity of the model in a trainable sense, giving careful consideration to the raw feature space and leveraging given resources, e.g., observed transcripts can be crucial.


% \section{Implementation details}
% \label{implementation details}
% \begin{algorithm}
% \small
% \caption{single-cell Feature Propagation (scFP)}\label{alg:scFP}
% \hspace*{\algorithmicindent} \textbf{Input:} Cell-Gene Matrix $\mathbf{X}$, Initial $k$NN $\tilde{\mathbf{A}}^{\text{initial}}$\\
% \hspace*{\algorithmicindent} \textbf{Output:} Denoised Cell-Gene Matrix $\tilde{\mathbf{X}}$
% \begin{algorithmic}[1]
% \State $\mathbf{Y} \gets \mathbf{X}$
% \While{$\mathbf{X} \text{ has not converged}$}
% \State $\mathbf{X} \gets \tilde{\mathbf{A}}^{\text{initial}}\mathbf{X}$
% \State $\mathbf{X}_{k,d} \gets \mathbf{Y}_{k,d} \forall k \in \mathcal{V}_{k,d}, \forall d \leq M$ \Comment{Hard Clamping}

% \EndWhile

% \State $\tilde{\mathbf{A}}^{\text{refined}} = k\text{NN}(\mathbf{X}^{(K)})$ \Comment{Refine $k$NN}

% \While{$\mathbf{X}^{(K)} \text{ has not converged}$} 
% % \State $\mathbf{X} \gets \tilde{\mathbf{A}}^{\text{refined}}\mathbf{X}$
% % \State $\mathbf{X}_{k,d} \gets \mathbf{Y}_{k,d} \forall k \in \mathcal{V}_{k,d}, \forall d \leq M$
% \State $\mathbf{X}^{(K)} \gets \alpha\tilde{\mathbf{A}}^{\text{refined}}\mathbf{X}^{(K)}+(1-\alpha)\mathbf{X}^{(K)}$ \Comment{Soft Clamping}

% \EndWhile

% \end{algorithmic}
% \end{algorithm}

% Observing that Equation~\ref{eqn:hard_fp} in Hard Feature Propagation essentially propagates features (i.e., gene expressions) via neighbors and resets the originally expressed gene values, we formulate the whole process in Algorithm~\ref{alg:scFP}. For the iteration until convergence, we used 40 as enough to converge, as mentioned in FP \cite{fp}. It is important to note that we did not use any trainable parameters during the whole process and obtained a denoised matrix solely by raw feature space. Overall, in this work, we aim to emphasize simple and straightforward ways to enhance performance in imputation on subsequent downstream tasks, e.g., cell clustering.









% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% \end{document}


% % This document was modified from the file originally made available by
% % Pat Langley and Andrea Danyluk for ICML-2K. This version was created
% % by Iain Murray in 2018, and modified by Alexandre Bouchard in
% % 2019 and 2021 and by Csaba Szepesvari, Gang Niu and Sivan Sabato in 2023. 
% % Previous contributors include Dan Roy, Lise Getoor and Tobias
% % Scheffer, which was slightly modified from the 2010 version by
% % Thorsten Joachims & Johannes Fuernkranz, slightly modified from the
% % 2009 version by Kiri Wagstaff and Sam Roweis's 2008 version, which is
% % slightly modified from Prasad Tadepalli's 2007 version which is a
% % lightly changed version of the previous year's version by Andrew
% % Moore, which was in turn edited from those of Kristian Kersting and
% % Codrina Lauth. Alex Smola contributed to the algorithmic style files.

